Automated Instantiation of Control Flow Tracing Exercises

One of the first steps in learning how to program is reading and tracing existing code. In order to avoid the error-prone task of generating variations of a tracing exercise, our tool Tatsu generates instances of a given code skeleton automatically. This is achieved by a finite unwinding of the program in the style of bounded model checking and using the SMT solver Z3 to find models for this unwinded program.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{J. Marcos, W. Neuper and P. Quaresma (Eds.): Theorem Proving Components\\ for Educational Software 2021 (ThEdu'21)\\
EPTCS 354, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.354.4}{10.4204/EPTCS.354.4}}
\pdfoutput=1

